Performance Analysis of Scientific Computing Workloads on Trusted Execution Environments

Scientific computing sometimes involves computation on sensitive data. Depending on the data and the execution environment, the HPC (high-performance computing) user or data provider may require confidentiality and/or integrity guarantees. To study the applicability of hardware-based trusted execution environments (TEEs) to enable secure scientific computing, we deeply analyze the performance impact of AMD SEV and Intel SGX for diverse HPC benchmarks including traditional scientific computing, machine learning, graph analytics, and emerging scientific computing workloads. We observe three main findings: 1) SEV requires careful memory placement on large scale NUMA machines (1$\times$$-$3.4$\times$ slowdown without and 1$\times$$-$1.15$\times$ slowdown with NUMA aware placement), 2) virtualization$-$a prerequisite for SEV$-$results in performance degradation for workloads with irregular memory accesses and large working sets (1$\times$$-$4$\times$ slowdown compared to native execution for graph applications) and 3) SGX is inappropriate for HPC given its limited secure memory size and inflexible programming model (1.2$\times$$-$126$\times$ slowdown over unsecure execution). Finally, we discuss forthcoming new TEE designs and their potential impact on scientific computing.

==> distributed.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{Beyond Single Node}
Scientific computing workloads often scale across multiple machines (nodes).
In this work, we mainly focus on a single node to evaluate the performance of TEEs.
We did a preliminary investigation of the available support to enable TEEs across multiple nodes.
We tried to set-up a straw-man multi-node system with support of AMD SEV on CloudLab~\cite{Duplyakin+:ATC19}.
Although, current HPC systems mostly rely on high performance transport protocols like RDMA for communication among multiple nodes, our experiments showed that the current Mellanox's RDMA driver does not support the use of RDMA inside SEV enabled virtual machines.
Instead, we relied on TCP for communication among machines and experimented using OSU MPI microbenchmarks.
For point-to-point bandwidth benchmarks, we observed a bandwidth of 25Gbps and 12 Gbps (for 2MB data packets) for QEMU and QEMU+SEV versions (a difference of nearly 2$\times$).
However, latency remains the same (approximately 1000 $\mu$s) for both QEMU and QEMU+SEV (ranging from 1 byte to 2MB packet sizes).
It should be noted that the communication between nodes still happens in clear (as there is no support for encrypted communication between multiple nodes in SEV).
A naive solution to make this communication secure is to use a VPN connection.
We experimented with OpenVPN and found the slowdown of VPN based secure communication to be large.
For example, for point-to-point OSU microbenchmarks, the bandwidth number drops to approximately 1Gbps and
latency increases to 20000 $\mu$s in comparison to less than 1000 $\mu$s for a data packet size of 2MB.

Therefore, we conclude that there is a need to develop more performant architectures to enable TEEs across multiple nodes in a distributed memory system or in accelerator based systems.
There are some existing software based solutions to enable encrypted communication across nodes, but they might not be sufficient for scientifc computing scale workloads.
For example, SCONE~\cite{arnautov2016scone} provides a network shield which transparently protects the communication among multiple nodes (each with its SGX hardware).
Asylo~\cite{asylo} (open-source framework for developing enclave applications) allows enclave based applications to be scaled across multiple machines using gRPCs (google remote procedure calls).
Since Asylo~\cite{asylo} is agnostic of TEE implementation, it can help in the scaling of both SGX and SEV based applications.

\begin{comment}
\subsection{TEEs in Accelerator Based Systems}
Examples of research works to enable trusted execution in accelerator based systems include:
Graviton~\cite{volos2018graviton} and HETEE~\cite{hetee}.
Graviton~\cite{volos2018graviton} provides trusted execution capabilities on GPUs by providing isolation to sensitive kernels from other code executing on GPUs and the host.
HETEE~\cite{hetee} relies on a centralized controller to manage trusted execution on all computing units including GPUs and accelerators.
However, there is still a need to investigate what new features need to be added to existing practical TEE solutions to enable trusted execution in accelerator based systems.
\end{comment}

\subsection{Observations on Security of TEEs}
Although the focus of this paper is the performance analysis of TEEs for secure HPC, it might be useful to readers to provide a brief security analysis of TEEs discussed in this paper.
SGX provides integrity guarantees while SEV lacks such support.
However, SEV is conisdered to be good enough by Google's confidential cloud computing initiative.
Also, new variations of SEV have been introduced to provide integrity support as well.
AMD has introduced  SEV-ES~\cite{amd:seves} that adds encryption of guest register state
to provide additional protection against VM state related attacks, and SEV-SNP~\cite{amd:sevsnp}
that  provides integrity checks.
These are encouraging developments from the security perspective,
as they address some of the vulnerabilities and limitations of SEV.
It should be noted that SEV-SNP~\cite{amd:sevsnp} does not provide integrity gaurantees using merkle tree like data structures (as SGX does), therefore, it is more scalable and can support larger secure memory sizes (thus leading to better performance).
Going forward, Intel has plans for the next generation SGX~\cite{xing2016intel} that will allow dynamic
memory allocation to overcome the limited size of the EPC today, but systems based on so-called SGX2
are still not widely (if at all) available.
Instead, it seems Intel is also moving in the direction of full memory
encryption and virtual machine-based trusted execution environments like AMD's SEV with total memory encryption (TME) and multi-key total memory encryption (MKTME) technologies~\cite{intel:memencrypt,intel:tme}.

Finally, we would like to point out that the entire workflow of running a workload securely might involve other steps as well (like a secure connection to the computing resources) in addition to running it inside an SEV or SGX enclave.
However, we believe that the execution of the workload itself in a secure enclave is the most important factor for performance analysis.

==> future_outlook.tex <==
\section{Future Outlook and Research Avenues}
%\Outline{[Note: Adding some references to related work here, not sure if that's the right thing.]}
%In this section, we identify few future research directions to make TEEs more practical for HPC environments.
%This is not an exhaustive list of possible research avenues.

\subsection{Research Avenues for Software Frameworks}
\label{sec:avn-sw}
\textbf{\textit{Intelligent job scheduling:}} As discussed earlier, security requirements of HPC workloads are diverse.
At the same time, the HPC platforms can be heterogeneous possibly composed of nodes from multiple vendors e.g., Intel and AMD, thus making both SGX and SEV available in the same environment.
Therefore, we propose an intelligent job scheduler which can allocate applications to an appropriate node depending on their sensitivity and the expected slowdown from the secure environment.
The sensitivity of the workload can be fed to the scheduler from the user and the expected slowdown can be calculated using pre-trained models.
As a proof of concept, we train a second-degree regression model to predict the slowdown of workloads under SGX and SEV, using only the features from normal execution of programs.
We can achieve a mean square error of \num{2.81e-11} and \num{2.54e-6} for SGX and SEV respectively (an R2 score of 0.99).
The features (normalized to per million instructions) used in both of these models include: resident\_memory, native\_time, syscalls, loads, and mem\_accesses for SGX and  native\_time, L2\_TLB\_misses,  and mem\_accesses for SEV respecitively in the order of the highest to lowest observed correlation (with the slowdown).
For SGX, the highest correlation with slowdown is shown by resident\_memory feature which is directly related to EPC faults which appears to be the primary reason for SGX slowdowns (section~\ref{sec:sgxperf}).
In case of SEV, the second highest correlation with slowdown is shown by L2\_TLB\_misses (page table walks) feature which is directly related to KVM exits which seems to be the main reason for SEV slowdowns (section~\ref{sec:sevperf}).

\begin{comment}
\begin{table}[htbp]
  \centering
     \caption{Features used for ML model}
    \begin{tabular}{|p{4cm}|p{4cm}|}
    \Xhline{2\arrayrulewidth}
    \cellcolor{brown!25} \textbf{SGX} & \cellcolor{brown!25} \textbf{SEV} \\ \Xhline{2\arrayrulewidth}
    \cellcolor{brown!25} resident\_memory, native\_time, syscalls, loads, mem\_accesses & \cellcolor{brown!25} native\_time, L2\_TLB\_misses, mem\_accesses \\ \Xhline{2\arrayrulewidth}
  \end{tabular}
  \label{tab:mlfeatures}
  \end{table}
\end{comment}

~The predicted slowdown for each benchmark, using the trained models, are shown (with x marks) in Figure \ref{fig:sgxperf} and \ref{fig:sevperf} for SGX and SEV respectively.
\begin{comment}
\small
\begin{multline}
  Slowdown  = (\num{1.74e+1})exec\_time\_normal + (\num{6.18e-2})\\resident\_memory - (\num{5.68e-5})syscalls +
  (\num{-5.392e-8})\\mem\_accesses + (\num{3.21e-10})load\_ops + \num{2.2e-4}
\end{multline}
\end{comment}
\normalsize
\newline
\noindent

\begin{comment}
\newline
\newline
\noindent
\textbf{\textit{Dynamic Migration of Application Segments:}}
Another research direction to explore is building of tools to shift sensitive functions or parts of the application transparently to enclaves at runtime.
Similarly, the outsourcing of unsecure parts of the application to (untrusted) accelerators or general cores to improve performance can be done transparently using tools (if developed).
%\item Challenges of Tensors scone and Python language implementations
\newline
\newline
\noindent
\textbf{\textit{KVM exit clustering for mitigating slowdown:}} By scanning and decoding upcoming instructions the hypervisor can identifying the ones that will cause a KVM exit.
Then a cluster of exiting instructions can be formed which can be executed all at once, ultimately reducing the overall exit rate and the cycles spend for saving/restoring the VM's state.
\end{comment}


\begin{comment}
\textbf{\textit{Other Ideas:}}
Following is a brief list of some other ideas that need to be investigated to ensure
\begin{itemize}
  \item A separate (more flexible) hardware interface to secure memory enabling fast accesses.
  \item Enclave aware policies for the rest of the system,
        so that the performance guarantees (for other workloads) are not affected.
  \item Hardware support for partitioning an application across multiple secure enclaves. % - HASP 2019 paper \cite{chakrabarti2019scaling} – how that can work in general?
  \item	Secure MPI (message passing interface).% (what is the state-of-the-art? Is it going to be a big challenges? What needs to be encrypted?)
\end{itemize}

\subsection{Research Avenues for Users}

\textbf{\textit{Workload Slowdown Estimation:}}
Our work presents the slowdown of secure execution for three different benchmarks which are representative of the traditional HPC workloads.
This study can serve as the basis of slowdown estimation for other larger HPC applications.
For example, if a user has a workload which is largely composed of kernel functions similar to the ones studied in our work,
similar slowdown should be expected as shown in Figure \ref{fig:sgxperf} and \ref{fig:sevperf}.
\\
\noindent
\textbf{\textit{TEEs in Synergy with Other Secure Environments:}}
From the user's perspective, another direction that can be explored is the use of trusted execution environments with other existing secure environemnts to build agile secure frameworks.
For example, as BlockChain ensures integrity but does not guarantee confidentiality of the data, it can be used with trusted execution environment like SEV (which provides confidentiality but not integrity)
to build performant secure solutions for HPC environments.
\end{comment}

==> other_observations.tex <==
% \subsection{\textbf{Finding 4:} \ul{There exist some solutions to enable application scaling across nodes}}
% %\vspace{-1mm}
% HPC workloads often scale to multiple nodes.
% It is important to find out if TEE based secure execution of HPC workloads support scaling across multiple nodes.
% Intel SGX SDK does not provide support for scaling SGX applications across nodes, however, there exist multiple third-party solutions.
% For example, SCONE~\cite{arnautov2016scone} provides a network shield which transparently protects the communication among multiple nodes (each with its SGX hardware).
% Asylo~\cite{asylo} (open-source framework for developing enclave applications) allow enclave based applications to be scaled across multiple machines using gRPCs (google remote procedure calls).
% Since Asylo~\cite{asylo} is agnostic of TEE implementation, it can help in the scaling of both SGX and SEV based applications.
% Recently, an Intel SGX card \cite{chakrabarti2019scaling} has also been introduced to enable SGX on Intel's server platforms, which allows applications to be scaled across different processors on the card itself (and/or across cards).
% The communication across nodes is either done synchronously via TCP/IP network messaging (RPCs) or asynchronously via a shared memory region between the host and SGX cards.

% \begin{comment}
% \begin{figure}%[t]
%   %\centering
%   \subfloat{
%   \includegraphics[width=.5\textwidth]{figs/sev_perf.pdf}
%   }
%   %\subfloat[KVM exit rate]{
%   %\includegraphics[width=.5\textwidth]{figs/sev_kvm.pdf}
%   %	}
%   \caption{Performance Impact of SEV (x is predicted slowdown of the ML model (sec \ref{sec:avn-sw})) \vspace{-3ex}}
%   \label{fig:sevperf}
%   \end{figure}
% \end{comment}


==> related_work.tex <==
\section{Related Work}
\label{related}

There exist some studies \cite{Mofrad2018-hm, dinh2019everything, gottel2018security, Brenner2018-ek, ning2018preliminary, gottel2018security} on the performance impact of TEEs which either focus on a single TEE or a comparison of different TEEs.
These studies are different from our work in three fundamental ways: (1) none of these works focus on HPC, (2)they target micro-benchmarks or small benchmarks which are usually single-threaded, (3) with reference to SEV, none of these works seem to be targeting large machines with multiple NUMA nodes. 
Mofrad et al~\cite{Mofrad2018-hm} did a comparative study of Intel SGX and AMD SEV.
Experimental comparison in this work (using workloads like Quicksort, MD5 Hash Function, synthetic benchmark executing different floating point operations) indicates that the SEV has negligible performance overhead in comparison to the SGX's overhead (specially when input data size is large). 
Ngoc et el~\cite{dinh2019everything} did a study of Intel SGX on virtualized systems (using microbenchmarks, and some SSL and HTTP benchmarks) and showed that for memory-heavy benchmarks, performance of virtualized SGX can be improved significantly using shadow paging instead of nested paging, however, for benchmarks with many context switches shadow paging is worse than nested paging.  
Brenner et al~\cite{Brenner2018-ek} presented performance and security metrics to guide enclave application design. 
Using SGX with two services, SecureKeeper (secure version of Apache ZooKeeper) and Dumbledore (secure version of Voldemort key value store), they showed that using higher number of enclaves to run these applications (multiple threads in parallel) leads to decreased performance, as higher number of enclaves hits EPC memory limit and lead SGX driver to swap EPC pages. 
G\"{o}ttel et al~\cite{gottel2018security} studied performance and energy consumption differences of SGX and SEV using micro and macro-benchmarks (like Redis server, a publish/subscribe system) and concluded that SEV mostly showed near-native performance. 
In case of AMD SEV energy consumption matches the native case, while in SGX the energy consumption increases when the memory size is bigger than the EPC size.


Some papers have tried to survey multiple TEEs in general.
Maine et al~\cite{maene2017hardware} presented a survey of different hardware based trusted execution solutions from industry (TPM, TrustZone, SecureBlue++, SGX) and academia (AEGIS, Bastion, SMART, Sancus, Soteria, Iso-X, TrustLite, TyTAN, Sanctum).
Ning et al~\cite{Ning2017-nr} presented existing security challenges in TEEs and possible mitigation options.

There exist some research works that have tried to use TEEs to enable secure execution of certain HPC applications.
Genie~\cite{Zhangy2018-sq} is a solution for secure AI processing on medical data is proposed, which makes use of Intel SGX and ideas from blockchain technology.
Slalom~\cite{tramer2018slalom} makes use of TEEs to enable secure execution of sensitive operations of neural networks' inference, and outsources the computationally intensive operations are outsourced to an un-trusted processor.

Partitioning of applications into secure and non-secure parts is a difficult task, especially in HPC settings as HPC workloads often rely on various third-party libraries.
For instance, Lind et al. \cite{Lind2017-un} proposed Glamdring which is a framework for automatic application partitioning into secure and non-secure parts.

Some research works~\cite{taassori2018vault, Saileshwar2018-pu, Orenbach2017-ks} have tried to reduce the performance overheads of SGX by proposing improvements in its design.
Research by Taassori et al. \cite{taassori2018vault} introduced a variable arity integrity tree (VAULT) in SGX that results in a compact design with low depth and can enable larger sizes of secure memory.
Saileshwar et al. \cite{Saileshwar2018-pu} proposed a compact integrity tree that uses morphable counters rather than fixed-size counters to accommodate more counters in the same memory area.
The work of Orenbach et al. \cite{Orenbach2017-ks}, Eleos, which uses software-based address translation and management inside the enclave to eliminate the need of flowing out of the enclave in case of a page fault, helps to avoid exiting the enclave to handle EPC page fault (leading to lower performance overhead).

\begin{comment}
Similarly, there lies an opportunity to explore the dynamic remapping of pages rather than actually copying them from one memory type to another.
By learning the memory access pattern of applications, the sensitive pages can be prefetched in the secure memory from non-secure memory regions even before they are actually accessed, thus reducing the number of access faults.
Currently, before control is transferred to the kernel driver to handle EPC fault, lower 12 bits of CR2 register (holding the faulting virtual address) are cleared because of security concerns.
Thus the driver is not able to use those bits to help in predicting memory access patterns.
Moreover, Gjerdrum et al. \cite{gjerdrum2017performance} have shown the page fault handler to be over-eager and unable to utilize EPC exhaustively.
There lies an opportunity to enable kernel driver to use the application's memory access patterns to prefetch pages anticipated to be used or perform smart page eviction.
Similarly, the pre-fetching and page eviction can be handled entirely in the hardware making it part of the TCB.
\end{comment}

\begin{comment}
some other works:
Security in High-Performance Computing Environments
USING INTEL®SGX TECHNOLOGIES TO SECURE LARGE SCALE SYSTEMSIN PUBLIC CLOUD ENVIRONMENTS
On the Performance of Intel SGX
Preliminary Study of Trusted ExecutionEnvironments on Heterogeneous Edge Platforms
Security, Performance and Energy Trade-Offs of Hardware-Assisted Memory Protection Mechanisms.
Applications:
Using Trusted Execution Environmentsfor Secure Stream Processing of Medical Data
TensorSCONE: A Secure TensorFlow Framework Using Intel SGX.
heterogeneous environment:
TEEshift: Protecting Code Confidentiality bySelectively Shifting Functions into TEEs
Graviton: Trusted Execution Environments on GPUs.
Authentic Execution of Distributed Event-Driven Applications with a Small TCB.
Security Analysis of Encrypted Virtual Machines
Security analysis of AMD-SEV solution
Guest attacks: memory, state
Host attacks: Page table access
Replay attacks
SoK: A Study of Using Hardware-assisted Isolated Execution Environments for Security
General description of AMD mechanism
\end{comment}
